Proactively Reducing the Hate Intensity of Online Posts via Hate Speech Normalization

Curbing online hate speech has become the need of the hour; however, a blanket ban on such activities is infeasible for several geopolitical and cultural reasons. To reduce the severity of the problem, in this paper, we introduce a novel task, hate speech normalization, that aims to weaken the intensity of hatred exhibited by an online post. The intention of hate speech normalization is not to support hate but instead to provide the users with a stepping stone towards non-hate while giving online platforms more time to monitor any improvement in the user's behavior. To this end, we manually curated a parallel corpus - hate texts and their normalized counterparts (a normalized text is less hateful and more benign). We introduce NACL, a simple yet efficient hate speech normalization model that operates in three stages - first, it measures the hate intensity of the original sample; second, it identifies the hate span(s) within it; and finally, it reduces hate intensity by paraphrasing the hate spans. We perform extensive experiments to measure the efficacy of NACL via three-way evaluation (intrinsic, extrinsic, and human-study). We observe that NACL outperforms six baselines - NACL yields a score of 0.1365 RMSE for the intensity prediction, 0.622 F1-score in the span identification, and 82.27 BLEU and 80.05 perplexity for the normalized text generation. We further show the generalizability of NACL across other platforms (Reddit, Facebook, Gab). An interactive prototype of NACL was put together for the user study. Further, the tool is being deployed in a real-world setting at Wipro AI as a part of its mission to tackle harmful content on online platforms.

==> tables/tab_dataset_stat.tex <==
\begin{table*}
    \centering
    \begin{tabular}{l|c|c|c|c|c}
          & \multirow{2}{*}{No. of Tweets}  & \multicolumn{2}{c|}{Utterance Len} & \multicolumn{2}{c}{Spans} \\ \cline{3-6} 
         & & Avg & Max & Avg spans per tweet  & Avg Len of span  \\ \hline \hline
         Train & 1653 &23 & 113 & 2 & 3 \\
         Test & 1000 & 18 & 99 & 2 & 3  \\ \hline
    \end{tabular}
    \caption{Statistics for the train and test data }
    \label{tab:dataset:stat2}
    \vspace{-2mm}
\end{table*}

==> tables/tab_extrinsic_hate_detect_stats.tex <==
\begin{table}
    \centering
    
    \vspace{-.20cm}
    % \resizebox{\columnwidth}{!}
    {%
    \begin{tabular}{l|c|c}
          \multicolumn{1}{c|}{\textbf{Model}} & \textbf{\# of tweets} & \textbf{Hate:Non-Hate}\\ \hline
          \citet{waseem-hovy-2016-hateful} & 12772  & 4750:8022\\
          \citet{davidson2019racial} & 24783 & 20620:4183\\
          \citet{founta2018unified} & 59189 & 13551:45638\\ \hline
    \end{tabular}
    }
    \caption{The hate vs non-hate tweet ratio for the hate classification. The data is collected from the respective hate detection methods.}
    \label{tab:hate_detection_stats}
    %  \vspace{-2mm}
    % \vspace{-2mm}
\end{table}

==> tables/tab_human_evaluation.tex <==
\begin{table*}
    \centering
    \begin{tabular}{l|c|c|c}
           \multirow{2}{*}{Model} & \multicolumn{3}{c}{Human Evaluation}   \\ \cline{2-4}
         & Intensity  $\downarrow$ & Fluency $\uparrow$  & Adequacy $\uparrow$  \\ \hline \hline
         Dictionary Model & 2.190 & 2.701 & 3.091 \\ \hline
         FGSA & 2.687  & 4.081 & 3.618   \\ 
         Bias Neutralization & 3.270 & 3.157 & 3.602 \\ \hline
         
         \hline
         \bf HSR & 2.048  & 4.386 & 4.165  \\ \hline
    \end{tabular}
    \vspace{-2mm}
    \caption{ Average scores for the Human Evaluation of generated text from different models for strength reduction, based on hate strength, fluency and adequacy of the generated text.  $\downarrow$ means lower is better and vice versa.}
    \label{table}
    
\end{table*}

==> tables/tab_reddit.tex <==
 \begin{table*}
    \centering
    
    \vspace{-2mm}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|p{55em}|c}
   {\bf \#} & {\bf Type} & \hfil\bf{Reddit Posts} &\hfil\bf{Int} \\ \hline \hline
    1. & Org & {\em A subsection of \{\textcolor{blue}{retarded Hungarians}\}\textcolor{red}{$_{Span}$}? Ohh boy brace for a \{\textcolor{blue}{livid Bulbasaur}\}\textcolor{red}{$_{Span}$} coming in here trying to \{\textcolor{blue}{hate a hole in}\} some of her \{\textcolor{blue}{stupider countrymen}\}}\textcolor{red}{$_{Span}$} & 8 \\ \cdashline{2-4}
    & Norm & 
    {\em A subsection of people? Ohh boy brace for a livid person coming in here trying to hurt some of her countrymen} & 4  \\ \hline
    2. & Org & {\em jesus, this is the \{\textcolor{blue}{most retarded}\}\textcolor{red}{$_{Span}$} thread i've read in a while} & 6 \\ \cdashline{2-4}
    & Norm & {\em jesus, this is the worst thread i've read in a while} & 3    \\ \hline
    3. & Org & {\em I'll agree with that \{\textcolor{blue}{b**ch}\}\textcolor{red}{$_{Span}$} Rick, the \{\textcolor{blue}{couple fa**ots}\}\textcolor{red}{$_{Span}$} I know who say he's one of their favorite characters are \{\textcolor{blue}{insufferable twats}\}}\textcolor{red}{$_{Span}$} & 8 \\ \cdashline{2-4}
    & Norm &  {\em I'll agree on Rick, the couple people I know who say he's one of their favorite characters are unpleasant} & 4    \\ \hline
    % 
\end{tabular}}
 \caption{Cross-platform study of \name. Outputs of \name\ (trained on tweets) on hateful Reddit posts \cite{qian-etal-2019-benchmark}.}
    \label{tab:error:reddit}
 \vspace{-2mm}
\end{table*}  
 
